Realizing LLMs' Causal Potential Requires Science-Grounded, Novel Benchmarks

Recent claims of strong performance by Large Language Models (LLMs) on causal discovery are undermined by a key flaw: many evaluations rely on benchmarks likely included in pretraining corpora. Thus, apparent success suggests that LLM-only methods, which ignore observational data, outperform classical statistical approaches. We challenge this narrative by asking: Do LLMs truly reason about causal structure, and how can we measure it without memorization concerns? Can they be trusted for real-world scientific discovery? We argue that realizing LLMs' potential for causal analysis requires two shifts: (P.1) developing robust evaluation protocols based on recent scientific studies to guard against dataset leakage, and (P.2) designing hybrid methods that combine LLM-derived knowledge with data-driven statistics. To address P.1, we encourage evaluating discovery methods on novel, real-world scientific studies. We outline a practical recipe for extracting causal graphs from recent publications released after an LLM's training cutoff, ensuring relevance and preventing memorization while capturing both established and novel relations. Compared to benchmarks like BNLearn, where LLMs achieve near-perfect accuracy, they perform far worse on our curated graphs, underscoring the need for statistical grounding. Supporting P.2, we show that using LLM predictions as priors for the classical PC algorithm significantly improves accuracy over both LLM-only and purely statistical methods. We call on the community to adopt science-grounded, leakage-resistant benchmarks and invest in hybrid causal discovery methods suited to real-world inquiry.

==> covid19_small_results.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Metric} & \textbf{LLM Pairwise} & \textbf{LLM BFS} & \textbf{LLM Triplet} & \textbf{Our Approach} & \textbf{PC} & \textbf{GES} \\ 
\midrule
\textbf{Precision} & 0.26 & 0.75 & Value 3 & Value 4 & 0.23 & 0.16 \\
\textbf{Recall}    & 0.35 & 0.45 & Value 9 & Value 10 & 0.15 & 0.2 \\
\textbf{F1 Score}  & Value 13 & Value 14 & Value 15 & Value 16 & Value 17 & Value 18 \\
\bottomrule
\end{tabular}
\caption{Comparison of Precision, Recall, and F1 Score for different methods on COVID-19 dataset}
\label{tab:covid19_metrics_clean}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Metric} & \textbf{LLM Pairwise} & \textbf{LLM BFS} & \textbf{LLM Triplet} & \textbf{Our Approach} & \textbf{PC} & \textbf{GES} \\ 
\midrule
\textbf{Precision} & Value 1 & Value 2 & Value 3 & Value 4 & 0.11 & 0.25 \\
\textbf{Recall}    & Value 7 & Value 8 & Value 9 & Value 10 & 0.05 & 0.1 \\
\textbf{F1 Score}  & Value 13 & Value 14 & Value 15 & Value 16 & Value 17 & Value 18 \\
\bottomrule
\end{tabular}
\caption{Comparison of Precision, Recall, and F1 Score for different methods on COVID-19 non-linear dataset}
\label{tab:covid19_metrics_clean}
\end{table}

==> cut.tex <==
\begin{table}[th]
\centering
\caption{Zero-shot Prediction Analysis for ASIA (Lung Cancer) and Earthquake Datasets\amit{taken from CDSM. Numbers need to be updated}}
\begin{tabular}{lcccc}
\toprule
\textbf{Metric} & \textbf{ASIA (Lung Cancer)} & \textbf{Earthquake} & \textbf{Child} & \textbf{Cancer}  \\ \hline
\textbf{Number of nodes} & 8 & 5 & 20 & 5\\ 
\textbf{Number of arcs} & 8 & 4 & 25 & 4\\ 
% \textbf{Correctly predicted nodes} & 5  & 5  \\ \hline
\textbf{Recall for nodes} & 0.625 & 1.0 & 1 & 1 \\ 
% \textbf{Correctly predicted arcs} & 2  & 4  \\ \hline
\textbf{Recall for arcs} & 0.25  & 1.0 & 1 & 1 \\
\bottomrule
\end{tabular}
\end{table}


\begin{example}
Consider a language model trained on the following causal relationships: Rain causes wet grass; Sprinkler causes wet grass; Anything indoor is not affected by rain. Consider a novel graph constructed after the language model's training cutoff date. The graph includes three causal queries: 1) Does rain cause the grass to be wet?; 2) Does a cloudburst lead to damp grass?; 3) Does rain cause indoor grass to be damp?
\begin{enumerate}
\item \textbf{Retrieval-only:} The first question can be answered by simply retrieving the correct fact from the language model's training data.
\item \textbf{(Complex) Transformation + Retrieval}: The second question can be answered by first transforming \textit{cloudburst} and \textit{damp} to similar semantic words, rain and wet. After the transformation, the answer follows after using retrieval.
\item \textbf{Reasoning + Transformation + Retrieval}: The third example requires reasoning to apply a relevant causal fact retrieved from the training data. Based on the causal fact about indoor objects, The model needs to infer that the grass is indoor and thus rain should not affect it. In addition, some transformation is needed to convert \textit{damp} to its similar word, \textit{wet}.
\end{enumerate}
\end{example}



































\begin{table}[H]
\centering
\caption{Precision and Recall Scores of Different Algorithms on the Alzheimer's Dataset}
\label{tab:alzheimers_results}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Algorithm}      & \textbf{Precision} & \textbf{Recall}  \\ \hline
PC  & 0.21         & 0.157         \\ \hline
GES  & 0.263         & 0.263         \\ \hline
LLM Pairwise  & 0.17         & 0.31         \\ \hline
LLM BFS  & 0.15         & 0.15         \\ \hline
Ours  & 0.33         & 0.78         \\ \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\caption{Precision and Recall Scores of Different Algorithms on the Covid-19 Respiratory Dataset.}
\label{tab:respiratory_results}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Algorithm}      & \textbf{Precision} & \textbf{Recall}  \\ \hline
PC  & 0.23         & 0.15         \\ \hline
GES  & 0.16         & 0.2         \\ \hline
LLM Pairwise  & 0.26         & 0.35         \\ \hline
LLM BFS  & 0.75         & 0.45         \\ \hline
Ours  & 0.48         & 0.60         \\ \hline
\end{tabular}
\end{table}

\begin{comment}
\begin{table}[H]
\centering
\caption{Precision and Recall Scores of Different Algorithms on the Complications Dataset : Covid 19}
\label{tab:respiratory_results}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Algorithm}      & \textbf{Precision} & \textbf{Recall}  \\ \hline
PC  & 0.23         & 0.15         \\ \hline
GES  & -         & -         \\ \hline
LLM Pairwise  & -         & -         \\ \hline
LLM BFS  & 0.23         & 0.16         \\ \hline
Ours  & 0.14         & 0.24         \\ \hline
\end{tabular}
\end{table}
\end{comment}



==> rebuttal.tex <==
\begin{itemize}
    \item NOTEARS, CAMML
    \item ALCM
    \item people will ask us to compare to other hybrid algorithms. esp. the one proposed by abdulaal et al. (alzheimer graph authors)
    \item we should also compare to aniket's triplet and the PC+LLM idea in that paper
    \item add the refinement step to the PC+LLM algo where we remove edges. Ensure acyclicity.
\end{itemize}


\section{Experiments}
\begin{comment}
\subsection{Memorization}
\begin{itemize}
    \item \textbf{Models} GPT-4 (sep 21), Llama 3 8B, 13B, GPT 3.5 turbo
    \item bnlearn datasets -- Done for GPT-4, Dump bnlearn experiments in overleaf.
    \item Memorization for our dataset  
    \item Run memorization experiments for Alzheimers and covid-19 small on Llama 3 70B, GPT-4. 
\end{itemize}

\subsection{Baselines}
\begin{itemize}
    \item Methods: PC, GES, NOTEARS, LinGAM and variants, CAMML, FCI. -Ashutosh 
    \begin{itemize}
        \item CAMML(low priority), LinGAM, and FCI are pending. 
    \end{itemize}
    \item  LLM methods: Pairwise, BFS, Triplet
    \begin{itemize}
        \item All LLM models should have 2021 as the cut-off (GPT-4, Llama 3 70B, GPT 3.5) 
        \item GPT-4, Llama models (Gautham to check with Aniket/Amit)
        \item Dump the LLM predictions as as graph
        \item LLM BFS is a priority
    \end{itemize}
    \item Hybrid Methods
    \begin{itemize}
        \item BFS + p-value
        \item CAMML + Prior
        \item Causallearn with BackgroundKnowledge
    \end{itemize}
\end{itemize}

\subsection{Our Method}
    \begin{itemize}
        \item Bottleneck is LLM BFS graph predictions
        \item Run LLM+PC on each graph from previous LLM BFS experiments.
        \item Tuning with LLM BFS as reference for PC, and implementation of edge removal phase to boost precision.
    \end{itemize}
\end{comment}


\section{TODOs}
\begin{itemize}
    \item Check bnlearn for linear settings citation - Lokesh
\end{itemize}

\textbf{Pitch: }Focus on benchmark more. We propose novel benchmarks. Eveluate algorithms. We propose a novel benchmarks, training data cut-off. To compare PC, we created synthetic dataset. Initial analysis, and then our result. - Lokesh
\begin{itemize}
    LLMs as constraints for score based algos
    \item Merging LLMs + Data exists -- Causal Architect (https://arxiv.org/pdf/2306.16902v1) -- CAMML (web interface)
    Score based + PC
    \item Aniketh's approach - PC first and then orientation using LLM
\end{itemize}


% \textbf{ICML Idea (https://arxiv.org/abs/2308.08493)}
% Two prompts - (a) Does a cause b, (b) For the dataset Asia, given an initial edges, complete the rest.
% Metrics -- (a) Accuracy on completion task  (b) Accuracy on completion task - accuracy under (a) above  

% zero-shot prompts



\section{Experiments}
\begin{enumerate}
    \item Memorization experiments on bnlearn datasets and novel datasets - with Gautam GPT cut-off date 2021
    \item Benchmarking - Ashutosh (classical) Gautham (LLM with old models) Random Approach
    \item Hybrid Approach (Aniket, Bengio, CAMML with prior, ours-new)  - Aniketh/Ashutosh
    \item  Ablation using recent GPT (Low priority) (hope: even GPT 2023 could not recall) 
    \item Ablation of our approaches: Our old proposal, Our method without removal - Ashutosh 
\end{enumerate}


}Contributions
\begin{itemize}
    \item Novel graphs that are released after LLM cutoff date. Proof of memorization. Prompts to elicit evidence of unmemorized novel graph.
    \item Evaluation of LLM-based methods on this benchmark. INSIGHT: Most methods over-create edges.
    \item Generate non linear data, MLP
    \item Proposed CI-test based algorithm that does better.
\end{itemize}

Codebase: \url{https://github.com/srivhash/causal-discovery}
\begin{itemize}
\item  Some general way to process existing graphs and include new graphs. 
\item  Some common API to call different LLM-based and data-based algorithms. Bengio, our algorithm, causal-learn, new algo.
\end{itemize}

\begin{itemize}
\item  Survey of PC style algorithms
pc, ges algo working
fisherz linear test, assumptions
\item  LLM
pairwise : time complexity
bfs : n calls
triplet : 
TODO : L: 
\url{https://assets.amazon.science/8a/eb/2c42690c43e998c55a89dcbe3bab/score-matching-enables-causal-discovery-of-nonlinear-additive-noise-models.pdf}
\end{itemize}

